Novel way of evaluating $g_A$ quenching in $\beta^+$/EC decays : Introducing the Branching-Ratio Method (BRM)

The novel Branching-Ratio Method (BRM) for the determination of effective value $g_{\rm A}^{\rm eff}$ of the weak axial coupling $g_{\rm A}$ for forbidden non-unique (FNU) $\beta^+$/electron-capture(EC) decays is introduced. The method offers new possibilities for testing the fitness of nuclear Hamiltonians in modeling the physics of complex $\beta^+$/EC decays. The constraint of simultaneously reproducing the branching to $\beta^+$ and EC transitions offers an additional constraint in tackling the problem of $g_{\rm A}^{\rm eff}$ determination. In the BRM the ambiguity in the choice of the values of $g_{\rm A}^{\rm eff}$ and s-NME (small relativistic vector nuclear matrix element) is lifted when constraints of the branching ratios of $\beta^+$ and EC decays are applied. As an example, in the present work we apply BRM to the case of second FNU $\beta^+$/EC decay of $^{59}$Ni. This decay is treated with three different nuclear shell-model (NSM) Hamiltonians demonstrating the effects of different nuclear-structure aspects in application of the BRM.

==> extra.tex <==
\begin{table}[H]
\caption{KB3GPN Computed s-NME values (s-NME$_{1}$ and s-NME$_{2}$) which reproduce the experimental total BR of the  2$^{\rm nd}$ forbidden $\beta^+ + \rm EC$ decay branch of $^{59}$Ni. The respective $BR_{\beta^+/EC}$ are presented corresponding to the s-NME}
\centering
    \label{sNME-KB3GPN}
    \resizebox{0.50\textwidth}{!}{%
    \begin{tabular}{ccccc}
    \toprule
        g$^{\rm eff}_{\rm A}$ & sNME$_{\beta^+/EC}$(1) & BR$_{\beta^+/EC}$ & sNME$_{\beta^+/EC}$(2) & $BR_{\beta^+/EC}$ \\ \midrule
        0.45  & -0.07365$^{}_{}$ & 1.55$^{}_{}$e-6 & 0.02589$^{}_{}$ & 3.34$^{}_{}$e-9 \\
        0.6  & -0.07981$^{}_{}$ & 1.64$^{}_{}$e-6 & 0.01943$^{}_{}$ & 7.68$^{}_{}$e-9 \\
        %0.7  & -0.08388 & 1.70e-6 & 0.01509 & 1.23e-8 \\
        0.8  & -0.08793$^{}_{}$ & 1.75$^{}_{}$e-6 & 0.01073$^{}_{}$ & 1.82$^{}_{}$e-8 \\
        %0.9  & -0.09195 & 1.81e-6 & 0.00634 & 2.57e-8 \\
        1.0  & -0.09594$^{}_{}$ & 1.87$^{}_{}$e-6 & 0.00193$^{}_{}$ & 3.46$^{}_{}$e-8 \\
        %1.1  & -0.09992 & 1.93e-6 & -0.00251 & 4.52e-8 \\
        1.2  & -0.10386$^{}_{}$ & 1.99$^{}_{}$e-6 &  -0.00698$^{}_{}$ & 5.74$^{}_{}$e-8 \\
        %1.27 & -0.10660 & 2.03e-6 & -0.01012 & 6.68e-8 \\
         & sNME$_{\beta^+}$(1) & & sNME$_{\beta^+}$(2) & \\
        0.6 & -0.02426$^{}_{}$ & 9.52$^{}_{}$e-6 & 0.07611$^{}_{}$ & 8.23$^{}_{}$e-8 \\
        %0.7  & -0.02649 & 6.75e-6 & 0.07389 & 7.92e-8 \\
        0.8  & -0.02872$^{}_{}$ & 4.94$^{}_{}$e-6 & 0.07167$^{}_{}$ & 7.63$^{}_{}$e-8 \\
        %0.9  & -0.03095 & 3.74e-6 & 0.06945 & 7.36e-8 \\
        1.0  & -0.03317$^{}_{}$ & 2.91$^{}_{}$e-6 & 0.06723$^{}_{}$ & 7.10$^{}_{}$e-8 \\
        %1.1  & -0.03539 & 2.32e-6 & 0.06501 & 6.85e-8 \\
        1.2  & -0.03762$^{}_{}$ & 1.89$^{}_{}$e-6  & 0.06278$^{}_{}$ & 6.61$^{}_{}$e-8 \\
        %1.27 & -0.03917 & 1.65e-6 &  0.06122 & 6.45e-8 \\
        & \multicolumn{2}{c}{sNME$_{CVC}$=-0.115125671}  & & \\
        \bottomrule
    \end{tabular}}
\end{table}


\begin{table}[H]
\caption{FPD6PN Computed s-NME values (s-NME$_{1}$ and s-NME$_{2}$) which reproduce the experimental total BR of the  2$^{\rm nd}$ forbidden $\beta^+ + \rm EC$ decay branch of $^{59}$Ni. The respective $BR_{\beta^+/EC}$ are presented corresponding to the s-NME}
\centering
    \label{sNME-FPD6PN}
    \resizebox{0.50\textwidth}{!}{%
    \begin{tabular}{ccccc}
    \toprule
        g$^{\rm eff}_{\rm A}$ & sNME$_{\beta^+/EC}$(1) & BR$_{\beta^+/EC}$ & sNME$_{\beta^+/EC}$(2) & $BR_{\beta^+/EC}$ \\ \midrule
        0.6  & -0.04350$^{}_{}$   & 6.74$^{}_{}$e-8 &  0.05584$^{}_{}$ & 8.94$^{}_{}$e-7 \\
        %0.7 & -0.04282    & 6.47e-8 & 0.05620 & 8.97e-7 \\
        0.8 & -0.04210$^{}_{}$   & 6.19$^{}_{}$e-8 &  0.05655$^{}_{}$ & 8.99$^{}_{}$e-7 \\
        %0.9 & -0.04135   & 5.90e-8 &  0.05686 & 9.01e-7 \\
        1.0 & -0.04058$^{}_{}$   & 5.60$^{}_{}$e-8 &  0.05715$^{}_{}$ & 9.02$^{}_{}$e-7 \\
        %1.1 & -0.03977  & 5.30e-8 &   0.05741 & 9.02e-7 \\
        1.2 & -0.03894$^{}_{}$  & 4.99$^{}_{}$e-8 &   0.05764$^{}_{}$ & 9.02$^{}_{}$e-7 \\
        %1.27 & -0.03835   & 4.78e-8 &  0.05778 & 9.01e-7 \\
         & sNME$_{\beta^+}$(1) & & sNME$_{\beta^+}$(2) & \\
        0.6  & -0.07244$^{}_{}$  & 1.50$^{}_{}$e-7 & 0.02799$^{}_{}$ & 1.75$^{}_{}$e-6 \\
        %0.7 & -0.07219    & 1.49e-7 & 0.02823 & 1.74e-6 \\
        0.8 & -0.07194$^{}_{}$    & 1.47$^{}_{}$e-7 &  0.02847$^{}_{}$ & 1.72$^{}_{}$e-6 \\
        %0.9 & -0.07169    & 1.46e-7 &  0.02871 & 1.69e-6 \\
        1.0 & -0.07144$^{}_{}$    & 1.44$^{}_{}$e-7 &  0.02895$^{}_{}$ & 1.66$^{}_{}$e-6 \\
        %1.1 & -0.07120    & 1.42e-7 &  0.02918 & 1.62e-6 \\
        1.2 & -0.07094$^{}_{}$    & 1.41$^{}_{}$e-7 & 0.02942$^{}_{}$ & 1.57$^{}_{}$e-6 \\
        %1.27 & -0.07077   & 1.40e-7 &   0.02958 & 1.53e-6 \\
        & \multicolumn{2}{c}{sNME$_{CVC}$=0.0692797750}  & & \\
        \bottomrule
    \end{tabular}}
\end{table}
